Distribution Aware Metrics for Conditional Natural Language Generation

Traditional automated metrics for evaluating conditional natural language generation use pairwise comparisons between a single generated text and the best-matching gold-standard ground truth text. When multiple ground truths are available, scores are aggregated using an average or max operation across references. While this approach works well when diversity in the ground truth data (i.e. dispersion of the distribution of conditional texts) can be ascribed to noise, such as in automated speech recognition, it does not allow for robust evaluation in the case where diversity in the ground truths represents signal for the model. In this work we argue that existing metrics are not appropriate for domains such as visual description or summarization where ground truths are semantically diverse, and where the diversity in those captions captures useful additional information about the context. We propose a novel paradigm for multi-candidate evaluation of conditional language generation models, and a new family of metrics that compare the distributions of reference and model-generated caption sets using small sample sets of each. We demonstrate the utility of our approach with a case study in visual description: where we show that existing models optimize for single-description quality over diversity, and gain some insights into how sampling methods and temperature impact description quality and diversity.

==> sections/outline.tex <==

\clearpage
\section{Outline}
\label{sec:outline}

\begin{outline}
    \1 Introduction
    \1 Related Work
        \2 Existing Natural Language Metrics
            \3 BLEU, ROUGE, METEOR, BERT-Score, SPICE
            \3 CIDEr
            \3 Visual Description Specific
                \4 CLIP-Score
                \4 TIGEr/FAIEr
                \4 SMURF
        \2 Diversity Statistics
            \3 Zipf Coefficient
            \3 Self-BLEU
            \3 Generation Perplexity
            \3 Epsilon Perpleixty
            \3 Sparsemax score
            \3 Token JS-Div
        \2 HUSE
        \2 MAUVE
    \1 Methods
        \2 Kernel-Distance Metrics
            \3 Frechet-BERT Distance
            \3 MMD-BERT Distance
        \2 Triangle Rank Metrics
    \1 Case Study: Visual Description
        \2 Analysis: Model Evaluation
            \3 Evaluating diverse models (such as CLIP-cap, O2NA)
                \4 Diversity vs. Fluency
                \4 N-Samples Required
        \2 Analysis: Sampling Methods
            \3 Ranking sampling methods for visual description
            \3 The importance of temperature
                \3 Standard Metric Correlations over Temperature
        \2 Analysis: Human Leave one Out Performance vs. Model Performance
    \1 Case Study: Summarization
        \2 Evaluation of summarization models (\url{https://github.com/Yale-LILY/SummEval#evaluation-toolkit})
        \2 Interesting results?
    \1 Rank Metrics vs. Kernel Distance Metrics
        \2 Multi-Modal Semantic Distributions
        \2 Performance
    \1 Limitations
        \2 Ground Truth Availability
        \2 Limited Knobs for Evaluation (Exclusivity)
    \1 Conclusion
\end{outline}




\section{Notes}

There are several possible directions for this paper to take. First, I'll introduce the existing contributions, then, I'll look at the possible directions that the project could take en route to a submission.

\subsection{Contributions}

\paragraph{Captioning Paradigm} The current captioning paradigm, in use by papers such as O2NA \cite{liu2021o2na} is focused on generating a single key caption for each video segment. This has a key flaw: it assumes that there \textit{is} a single correct caption for each clip. In practice, as seen by several existing papers, even human references for a single clip can be highly variable. In this case, unlike in classification, \textbf{noise in the labels is information,  not variance}. This fact suggests that we should train captioning models to approximate a full distribution of possible text captions, rather than a single-best captioning model as is currently done. We have several existing experiments supporting these claims:

\begin{outline}
    \1 Experiments showing that existing captioning models are bad at approximating the full distribution
        \2 Poor performance of SOTA models at high sampling temperature
        \2 Highly degraded fluency of SOTA models at high sampling temperature
        \2 Poor diversity in beam-search based N-best lists
    \1 Experiments showing high semantic diversity within a single caption
    \1 Experiments showing that CIDEr/METEOR/BLEU/ROUGE are biased towards single highly relevant captions (previous work)
    \1 Experiments showing that the conditional information of the video given the generated captions is relatively low
    
\end{outline}

\paragraph{Distribution-Aware Metrics} Given the above shift in paradigm, we want to find a way to measure distributional correlation between the ground truths/reference metrics, and the generated candidate captions. There have been few works which focus on such distribution-level correlation, particularly in the NLP space. The closest work is \cite{pilluta2021mauve}, which attempts to measure open-ended text generation at a high level using distributional approximations. We have already generated several interesting distribution-aware metrics for evaluating text generation. We introduce several novel metrics based on this paradigm:

\begin{outline}
    \1 Metrics based on \cite{liu2011triangle} (rank-based statistics) using underlying distances from the traditional literature such as BLEU, METEOR, BERT Embedding Distance, etc.
    \1 Metrics based on measuring distances between estimated distributions
        \2 MMD-Based distributional distance (Gaussian or RBF kernel) distance
        \2 Frechet BERT distance (Estimate Frechet distance between independent gaussian feature estimates)
\end{outline}

\subsection{Directions}

\paragraph{Novel Models} One of the things that we have noticed using our metrics, is that as we increase the sampling temperature to improve the diversity of the input samples, there is a great breakdown in the fluency of the models. One possible direction for this work is to introduce a novel model, which improves fluency at the higher diversity temperatures (thus decreasing our metric, while keeping CIDEr/etc. similar). This would demonstrate the reason for using our metric, but could also be difficult to complete. We have several existing possibilities (i.e. code already written) for such a model:

\begin{outline}
    \1 A model which leverages a frozen pre-trained language model in some capacity:
        \2 Distilling the pre-trained language model into the existing model
        \2 Using a frozen version of the pre-trained language model and tuning the prefix inputs
    \1 A model which leverages some amount of de-biasing on the input. Such models would be able to decrease the expected conditional variance of the output captions, and thus, perform better when approximating the output distributions.
        \2 Models which have some amount of noise specified in the input space
        \2 Model which do some amount of self-supervised summarization prior to the outputs.
    \1 A model which trains directly on one of our metrics above (or is fine-tuned on one of those metrics)
\end{outline}

To realize this concept, we would need to do the following:
\begin{outline}
    \1 Find a model which is similarly performant on CIDEr score to a SOTA method
    \1 Show that this model also improves diversity
\end{outline}

This is, perhaps, the most complicated of the possible approaches, since it requires finding a unique insight, and applying that insight in the next few weeks.

\paragraph{Existing Models} Another possible direction to explore would be to re-evaluate existing models using our metric paradigms, and show that our metric can break ties, particularly in the diversity space. To realize this direction we would need to:

\begin{outline}
    \1 Expand the number of other models we are testing (currently only O2NA is evaluated)
        \2 Challenge: A lot of code isn't available, or doesn't work
    \1 Show that rankings change when certain choices are made
        \2 Challenge: This is mostly up to chance, but hopefully something will appear in terms of possible directions and analysis.
\end{outline}

This is a technically much simpler direction to take than generating our own model, however requires a fair amount of literature work, and the ability to generate test-time samples from a number of different models. This can often be relatively challenging, as the existing models either don't have code, or don't provide an ability to extract test-time samples directly. We already had to modify O2NA to allow for test-time sampling (as opposed to single-best sampling).

\paragraph{Smaller Tricks} We could also demonstrate the utility of our metric as it pertains to smaller trick, such as swapping synonyms and other basic metric choices. This is actually something that I think that we should probably do regardless, to attempt to help the readers understand exactly how the metrics are impacted by certain choices, and allow the readers to gain some intuition about how the metrics function in practice. 

\paragraph{Evaluating Sampling Methods} We can demonstrate the performance of our model on several different sampling methods, which could yield better performance. There are several things that we could do here:
\begin{outline}
    \1 Demonstrate the ordering between sampling and decoding methods
    \1 Introduce a new sampling/decoding method that improves on our metric, yet yields different details on baseline methods.
\end{outline}

We already have the following methods implemented:
\begin{outline}
    \1 Sampling (with arbitrary temperature)
    \1 Beam Search (and sampled beam search)
    \1 Nucleus Sampling
    \1 Greedy Sampling
\end{outline}

In order to realize this direction, we would have to do the following:
\begin{outline}
    \1 Add some additional interesting decoding methods, which could add some diversity to our approach
        \2 Possible Method: Delorean
        \2 Possible Method: Diverse re-sampling based on language models
\end{outline}

It would actually be most interesting to leverage this in combination with one of the other directions here, as it's a somewhat quick experiment that would be best combined with a detailed exploration of the existing work, or with a new model introduction.

\paragraph{Other Tasks} There are several possible tasks which this model could be expanded to, including general conditional language generation (such as in \cite{pilluta2021mauve}), summarization etc. 

\section{Issues}

\paragraph{Fluency $>>$ Diversity?} One of the major issues that is facing our work is that there is an inherent trade-off in our metric between diversity and fluency. Fluent methods will perform well, but diverse methods will also perform well. Currently, even having fluent and diverse, but relatively off-topic sentences can improve on our metric (since current models are hyper-optimized for fluency over diversity), which can make it difficult to recommend our metric as a single solution to the problem (i.e. optimize this). 

\subsection{Additional Tasks}

\paragraph{Detailed Comparisons} Looking over the reviews of the MAUVE paper (\url{https://openreview.net/forum?id=Tqx7nJp7PR}), it seems like one thing that the reviewers requested are more detialed comparisons between the metrics. It would be useful to understand how we differ, and what the correlations between the metrics look like for different models. Regardless of the completion direction that we take, we should consider plots which present correlation between our metrics, and other SOTA metrics for visual description and conditional language generation tasks. The following metrics could be interesting to compare to:

\begin{outline}
    \1 Standard Metrics
        \2 BLEU
        \2 METEOR
        \2 ROUGE
        \2 CIDEr
        \2 SPICE
    \1 Modern Metrics
        \2 TIGEr
        \2 BERT-Score
        \2 CLIP-Score
        \2 SMURF
    \1 Distributional Metrics
        \2 MAUVE \cite{pilluta2021mauve}
        \2 HUSE \cite{hashimoto2019unifying}
    \1 Standard Diversity Metrics
        \2 N-Gram diversity
        \2 Vocab size
        \2 EVS (from our paper)
        \2 Reverse BLEU
\end{outline}

It would also be interesting to look at level-sets of these metrics across each other, and perhaps across different methods, to see what is working best, and what could continue to show improvement. 


==> sections/related.tex <==
\section{Related Work}
\label{sec:related}

This work is not the first to notice difficulties with traditional metrics for the automated evaluation of conditional language generation models. In visual dialog, \citet{caglayan2020curious} find that a number of the automated metrics proposed for visual dialog do not match well with human judgment, while in visual description, \citet{chan2022s} find that current automated metrics do not assign high scores to human-generated descriptions. This work not only quantifies such issues, but proposes a method for addressing these cases without developing novel metrics for measuring text semantic distance. 


Indeed, there is no shortage of automated metrics available to evaluate the semantic similarity between a single generated text to one or more human-written reference texts. The evaluation of machine-generated text has long been an active area of research,  which has continuously evolved to keep pace with accelerating advances in text generation models.
As a consequence of the tools available and the state of early text generation approaches, classical measures have primarily focused on evaluating the quality of generated text using surface-level text statistics. Most notably, these include $n$-gram matching based metrics like BLEU~\cite{papineni2002bleu}, METEOR~\cite{banerjee2005meteor}, ROUGE~\cite{lin2004rouge}, and CIDEr~\cite{vedantam2015cider}.

More recently, progress enabled by large-scale language models has motivated evaluation measures which go beyond n-gram statistics and toward linguistic semantics
~\cite{shimanaka2018ruse,clark2019sentence,zhang2019bertscore,sellam2020bleurt}. 
These approaches leverage high dimensional representations of generated and reference text provided by an external state-of-the-art language model, such as BERT~\cite{devlin2018bert} in the case of BERTScore~\cite{zhang2019bertscore} and BLEURT~\cite{sellam2020bleurt}.

The diversity of the generated text is often evaluated separately from the quality of the generated text. In fact, many common diversity measures only quantify surface level frequency statistics of the generated text, such as metrics based on the number of unique tokens, unique sentences, or unigram frequency statistics, as in the case of Zipf coefficients ~\cite{holtzman2019curious}. Some more complex measures, such as $n$-gram-based diversity measures are offered by metrics like self-BLEU~\cite{zhu2018texygen}, which computes BLEU scores between samples from a model. While such measures can quantify the diversity of the generated samples, they do not measure the diversity with respect to the diversity of the reference samples, leaving them vulnerable to over-optimizing for diversity when no diversity is required, or optimizing diversity at the cost of correctness or fluency.

Recently, MAUVE, proposed by \citet{pilluta2021mauve}, addresses the single-utterance evaluation paradigm by measuring the divergence between multi-candidate samples and multiple ground truths using density estimates in a text embedding space. Unfortunately, while MAUVE works well in scenarios when a large number of references are available, it does not work well when only a few references are available (due to its K-means distributional approximation) (see appendix \ref{app:mauve}). Such a low-reference scenario is common in conditional NLG, making MAUVE unsuitable for many applications.


% Indeed, there is no shortage of automated metrics available to evaluate the semantic similarity between a single generated utterance to one or more human-written reference utterances. These metrics can be roughly divided into automatic rule-based evaluation measures~\cite{papineni2002bleu,banerjee2005meteor,vedantam2015cider,lin2004rouge,anderson2016spice}, model-based evaluation measures~\cite{clipscore,tiger,smurf,pilluta2021mauve}, and separate diversity measures such as $n$-gram diversity and Zipf coefficients \cite{holtzman2019curious}.

% % Quality/Accuracy Focused Metrics 
% Rule-based evaluation measures directly compare the generated and reference text in terms of text n-gram matches. BLEU~\cite{papineni2002bleu}, METEOR~\cite{banerjee2005meteor} and ROUGE~\cite{lin2004rouge} compute scores based on n-gram precision and recall between generated and reference text, whereas,  CIDEr~\cite{vedantam2015cider} uses TF-IDF to measure n-gram similarity. Given multiple reference captions the standard approach has been to report the min, max or average of these scores over all references. 

% Model-based evaluation measures try to go beyond exact n-gram matches and instead try to evaluate at a higher semantic level. CLIPScore~\cite{clipscore} uses the CLIP~\cite{clip} model, a cross-modal retrieval model trained on 400M
% (image, caption) pairs gathered from the web, to extract embeddings for the generated caption and the input image and uses the cosine similarity between the two to compute a metric. CLIPScore is reference-free because it does not require any reference captions. RefCLIPScore~\cite{clipscore} extends the CLIPScore by incorporating the cosine similarity between the generated caption and the reference text along with the standard CLIPScore. TIGEr~\cite{tiger} uses a model to first compute a grounding vector that matches different parts of a caption with regions in the image. The final score is then computed as the similarity between the grounding vectors of the generated caption and the reference caption. SMURF~\cite{smurf} decomposes caption evaluation into the dimensions of semantics and fluency. SMURF computes a reference-free fluency metric called linguistic typicality using an attention-based information flow function estimated using a transformer. The semantic score is computed as a modified version of the F1 score of the concepts in the generated caption with respect to reference captions that incorporates the typicality function.   

% Diversity Focused Metrics

% All of these measures are largely designed to compute the distance between a single candidate utterance, and one or many reference utterances, and do not handle the situation in which several candidate utterances are proposed. Recently, MAUVE, proposed by \citet{pilluta2021mauve}, aims to change this by measuring the divergence between two samples in the text distribution space. Unfortunately, while MAUVE works well in scenarios when a large number of references are available, it does not work well when only a few references are available (due to it K-means distributional approximation) (see appendix \ref{app:mauve}). Such a low-reference scenario is common in conditional natural language generation, making MAUVE unsuitable for our application. 



==> sections/summarization.tex <==
\section{Case Study: Summarization}
\label{sec:summary}

The metrics we present here are also interesting in the context of automated summarization, where the goal is to produce a small summary of a longer natural language passage. Much like the visual description task, automated summarization is unique in that there is a high level of output diversity, however most summarization models are still evaluated using existing sample-wise natural language metrics.  Recently, \CN collected more than one ground truth summary for the CNN-DailyMail \CN summarization dataset, which allows us to explore the performance of several models on this new data. Table \TODO shows an evaluation of our metrics on several recent summarization models. As we can see \TODO. 
